Facilitating Database Tuning with Hyper-Parameter Optimization: A Comprehensive Experimental Evaluation

Recently, using automatic configuration tuning to improve the performance of modern database management systems (DBMSs) has attracted increasing interest from the database community. This is embodied with a number of systems featuring advanced tuning capabilities being developed. However, it remains a challenge to select the best solution for database configuration tuning, considering the large body of algorithm choices. In addition, beyond the applications on database systems, we could find more potential algorithms designed for configuration tuning. To this end, this paper provides a comprehensive evaluation of configuration tuning techniques from a broader perspective, hoping to better benefit the database community. In particular, we summarize three key modules of database configuration tuning systems and conduct extensive ablation studies using various challenging cases. Our evaluation demonstrates that the hyper-parameter optimization algorithms can be borrowed to further enhance the database configuration tuning. Moreover, we identify the best algorithm choices for different modules. Beyond the comprehensive evaluations, we offer an efficient and unified database configuration tuning benchmark via surrogates that reduces the evaluation cost to a minimum, allowing for extensive runs and analysis of new techniques.

==> R1.tex <==

   \begin{center}
      \Huge\textbf{Facilitating Database  Tuning with Hyper-Parameter Optimization: A Comprehensive Experimental Evaluation (Revision Cover Letter)}\\

   \end{center}
   \vspace*{1em}
   
We appreciate all the constructive comments and advice from the reviewers. We have carefully revised the whole paper and added substantial experiments in this revision, with the major modifications highlighted in \textcolor{blue}{blue}. 
We include additional analysis and experiments in Appendix due to the space constraint of the paper. 
In the following, we first summarize the major revisions and then respond to the reviewer with details. We add the original reviews before our response for each comment and mark the relevant paragraphs accordingly in the response.

\begin{table}[H]
\caption{Summary of major modifications.}
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Modifications}                                                                                                                                                                                                                                  & \multicolumn{1}{c|}{Corresponding Reviews}                              \\ \hline
\autoref{sec2.3}: Description of CGPTuner.                                                                                                                                                                                                          & REVIEWER\#1 D1                                                          \\ \hline
\autoref{sec:men-knob}, \autoref{sec:imple}:  Explicit statement abou Lasso’s disadvantage and its implementation.                                                                                                                 & REVIEWER\#1 D2                                                          \\ \hline
\autoref{sec:men-transfer}: Details about how fine-tune works.                                                                                                                                                                                      & REVIEWER\#1 D3                                                          \\ \hline
\autoref{sec4}: Explanation about the setting of buffer pool size.                                                                                                                                                                                  & REVIEWER\#1 D4                                                          \\ \hline
\autoref{sec:exp1-incremental}: Details about incremental knob selection.                                                                                                                                                                           & REVIEWER\#1 D5                                                          \\ \hline
\autoref{appendix}: Make the appendix~\cite{appendix} available online.                                                                                                                                                                                              & REVIEWER\#1 D7                                                          \\ \hline
\autoref{sec:exp2-performance}: Add one-hot BO as a baseline.                                                                                                                                                                                        & REVIEWER\#1 D8                                                          \\ \hline
\autoref{app:pg}: Experiments in PostgreSQL-- analyze important knobs and compare the optimizers.                                                                                                                                                   & REVIEWER\#2 W1                                                          \\ \hline
\begin{tabular}[c]{@{}l@{}}\autoref{sec:exp-tuning}: Explanation for choosing the two top ranking lists (Top-5 and Top-20).\\ \autoref{sec8}: Evaluation over the enumeration of all the ranking lists via surrogate.\end{tabular}                   & REVIEWER\#2 W2                                                          \\ \hline
\autoref{app-knob}: Add the top 20 configuration parameters selected by SHAP                                                                                                                                                                        & REVIEWER\#2 C1                                                          \\ \hline
\autoref{sec8}: Benchmark the knob selection modules.                                                                                                                                                                                               & REVIEWER\#2 C3                                                          \\ \hline
\autoref{app:pg-bench}: Tuning benchmark via surrogates in PostgreSQL.                                                                                                                                                                              & REVIEWER\#3 D1                                                          \\ \hline
\begin{tabular}[c]{@{}l@{}}\autoref{sec4}: Reasons for workload selection.\\ \autoref{sec:app-workload}:  Discussion about  the construction of transferring scenarios and representativeness of workloads.\end{tabular} & \begin{tabular}[c]{@{}l@{}}REVIEWER\#3 D2\\ REVIEWER\#3 D4\end{tabular} \\ \hline
Figure \ref{fig:exp1}: Box plot of importance measurements over all the underlying optimizers.                                                                                                                                                      & REVIEWER\#3 D3                                                          \\ \hline
\autoref{sec:exp2-performance}: Reference to existing macro evaluation.                                                                                                                                                                              & REVIEWER\#3 D5                                                          \\ \hline
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}




%\noindent\textbf{Note}: We include additional analysis and experiments in Appendix due to the space constraint of the paper. 
%The Appendix is available online\footnote{\url{https://github.com/DBoptimizer/OnlineTune/blob/main/Appendix_OnlineTune.pdf}}.

\section*{REVIEWER \#1}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D1: }\textit{This is another recent BO-based tuning tool to include (ideally in Section 2.3.1):
Stefano Cereda, Stefano Valladares, Paolo Cremonesi, and Stefano Doni.
CGPTuner: a Contextual Gaussian Process Bandit Approach for the Automatic Tuning of IT Configurations Under Varying Workload
Conditions. PVLDB, 14(8): 1401-1413, 2021.
}
\end{tcolorbox}
\noindent\textbf{Response: }
 Thanks for the suggestions.
 We include CGPTuner in \autoref{sec2.3} in the revised manuscript.
 
 \noindent\blue{``\textbf{CGPTuner~\cite{DBLP:journals/pvldb/CeredaVCD21}} proposes to  tune the configuration of an IT system, such as  the Java Virtual Machine (JVM) or the  Operating System (OS)) to unlock the full performance potential of a DBMS.
It adopts Contextual BO~\cite{DBLP:conf/nips/KrauseO11} to adapt  to workload variation, which requires an external workload characterisation module.''
}
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D2: }\textit{From what I understand, Lasso is the only knob selection algorithm that cannot detect nonlinear correlations between knobs. I think this is an important disadvantage and should be explicitly stated in Section 3.1. I would also be more specific in Section 4.2 and say that second-degree polymonial features are included to enable Lasso to detect interactions between pairs of knobs.
}
\end{tcolorbox}
\noindent\textbf{Response: }
We agree that it is necessary to explicitly state Lasso's disadvantage and its implementation.
We discuss the disadvantage of Lasso in \autoref{sec:men-knob}: \blue{``However, Lasso assumes the linearity of the knob space~\cite{krakovska2019performance} and is not able to  capture the non-linear dependencies from knobs to the performance metric.''}
And we modify the description of Lasso's implementation in \autoref{sec:imple}: 
\blue{``For Lasso~\cite{tibshirani1996regression}, we adopt the implementation in OtterTune which includes second-degree polynomial features to enable Lasso to detect interactions between pairs of knobs.''}
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D3: }\textit{In Section 3.3, please add some details about how Fine-tune works.
}
\end{tcolorbox}
\noindent\textbf{Response: }
As suggested by the reviewer, we add the details about how fine-tune works in \autoref{sec:men-transfer}: 
\blue{``For example, CDBTune and Qtune could pre-train a basic DDPG model by replaying historical workloads.
During the later practical use of the tuner, the tuner continuously gains feedback information of its recommendation for each user tuning request. 
It uses the feedback data to update its model by gradient descent (fine-tune).''}
% \blue{For example, CDBTune and Qtune could pre-train a basic DDPG model by replaying historical workloads, which is called offline tuning by CDBTune \cite{DBLP:conf/sigmod/ZhangLZLXCXWCLR19}.
% Later, once receiving a tuning request from a user, they use the model obtained by offline training to do further online tuning, since the user’s workload of the database in online tuning stage is different from the standard workload used for pre-training.
% Eventually, the knobs configuration corresponding to the best performance in online tuning will be recommended to the user.}
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}

\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D4: }\textit{In Section 4.1, can you quickly explain why you increase the buffer pool size from the MySQL default to 60\% memory for the experiments?}
\end{tcolorbox}
\noindent\textbf{Response: }
The MySQL default configuration for buffer pool size is 128 MB~\cite{MySQLKnob}, which severely limits the database performance.
And it is a common practise to set the buffer pool size 60\%\textasciitilde  80\% of RAM~\cite{MySQLBuffer}.
Since we want to compare with an reasonable default baseline, we increase the buffer pool size from the MySQL default to 60\% of the RAM for the experiments.
And we rewrite the description in \autoref{sec4} to better explain the setting: 
\blue{``And we use the MySQL default configuration as the default in our experiments except that we set a larger and reasonable buffer pool size (60\% of the instance's memory~\cite{MySQLBuffer}), since the default size (128 MB) in MySQL document largely limits the database performance.''}
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}

\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D5: }\textit{For the incremental knob selection experiments in Section 5.3, how often are you adding/removing knobs and how many knobs are adding/removing each time? This information is missing from the setup in 5.1.}
\end{tcolorbox}
\noindent\textbf{Response: }
For increasing the number of knobs, we begin  with tuning the top
four knobs and add two knobs  every four iterations.
For decreasing the number of knobs, we  begin with tuning all the knobs and remove 40\% knobs every 20 iterations.
The procedures are the same with OtterTune and Tuneful, except we decrease the knobs every 20 iterations instead of 10 iterations for Tuneful since we have more tuning budget (Tuneful's original setting leads to zero tuning knobs after 110 iterations).

Although this information is contained in the supplementary
material (i.e., the “KnobTuningEA\_Appendix.pdf”) submitted together with the paper, we agree it may confuse the readers upon the procedures of incremental knobs selection when reading the paper.
In the revised manuscript, we add this information in \autoref{sec:exp1-incremental}:
\blue{``For increasing the number of knobs, we begin  with tuning the\ldots''}
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}



\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D6: }\textit{ The setup in Section 6.1 says:
"... we use the configuration space of top-20 continuous knobs as a control group (continuous space) and the space of top-5 categorical knobs and top-15 integer knobs as a test group (heterogeneous space)."
}

\noindent\textit{
I would change "top-20 continuous knobs" -> "top-20 integer knobs" because when I first read this I thought you meant that the control group was made up of all numeric (real) knobs.}
\end{tcolorbox}
\noindent\textbf{Response: }
Thanks for the suggestion.
We change the description to ``top-20 integer knobs''  in the revised manuscript.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D7: }\textit{Sections 6.1, 7.1, and 8 mention additional results in the "Appendix" but this should reference your online artifacts instead.}
\end{tcolorbox}
\noindent\textbf{Response: }
As suggested by the reviewer, we make the appendix available online and refer to the online artifacts~\cite{appendix} in the revised manuscript.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}







\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D8: }\textit{For the experiments in Section 6.2, it sounds like you transform the categorical variables for Vanilla GP directly to integers (0 to n\_categories - 1), which is the naive approach. I would have liked to see one of the simple, well-known approaches for transforming categorical features used (e.g., one hot encoding). Including this experiment in 6.2.2 would make the comparison more complete and realistic.}
\textbf{W2: }\textit{The authors use the naive approach for transforming categorical variables when there are simple techniques frequently used with vanilla BO approaches to handle categorical variables that do not follow a natural ordering (e.g., one hot encoding).}

\end{tcolorbox}
\noindent\textbf{Response: }
We appreciate the reviewer’s comments on the baseline methods.
We add the BO baseline that transforms  categorical variables via one-hot encoding  (denoted as one-hot BO) in \autoref{sec:exp2-performance}.

The experimental results in Figures~\ref{fig:exp3} show that one-hot BO has a better performance than vanilla BO in most cases but is inferior to mixed-kernel BO.
This is because mixed-kernel BO also uses the one-hot encoding for categorical variables and adopts Hamming kernel to measure the distance of  categorical variables, better modeling the heterogeneity.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D9: }\textit{A non-exhaustive list of typos and presentations issues is below.\\
* Table 1: "ReIM" -> "RelM"\\
* Section 1.2: "paper.Next" -> "paper. Next"\\
* Section 2.2: "controller replay" -> "controller replays"\\
* Section 2.3.1: "workload encoder" -> "workload encoders"\\
* Section 2.3.2: "tuning, It" -> "tuning. It"\\
* Section 2.4: "It is common to use Gaussian process*es* (GP) as surrogates [56, 70]*,* and SMAC [34] and TPE [9] are *two other* well-established methods."\\
* Section 3.1.1: "variance of target" -> "variance of the target"\\
* Section 3.2: "In configuration" -> "In the configuration"\\
* Section 3.2: "i.g." -> "i.e." (2 occurrences)\\
* Section 3.2: "value of objective" -> "value of the objective"\\
* Section 3.2: "optimizations [65, 87]" -> "optimization [65, 87]."\\
* Section 4.1: "tuning sever" -> "tuning server"\\
* Section 5: "Q5.1", "Q5.2" -> "Q5.2", "Q5.3"\\
* Figure 3(a)/(c): "GP" -> "Vanilla BO" or "VBO"\\
* Section 6.2: "(action).However" -> "(action). However"\\
* Table 9: "Mixed-Kerenl" -> "Mixed-Kernel"\\
* Section 9.1: "prone" -> "prune"\\
* Some acronyms are introduced 2+ times throughout the paper, including "ML", "BO", "RL", "HPO", and "GP".\\
* Some instances of "e.g."/"i.e." are missing commas and/or parenthesis.}
\end{tcolorbox}
\noindent\textbf{Response: }
Thanks for the suggestion.
We have checked the manuscripts carefully and fixed the corresponding typos and presentation issues.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}

==> R2.tex <==

  \section*{REVIEWER \#2}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{W1: }\textit{ The paper does not show nor discuss whether their findings are transferable to other database systems (other than MySQL). I’m not suggesting repeating all experiments with another database system but perhaps replicate one experiment with another database system (e.g., PostgreSQL) to see whether the results are similar or not.
}
\end{tcolorbox}
\noindent\textbf{Response: }
We agree that it is meaningful to evaluate whether the findings are transferable to other database systems.
As suggested by the reviewer, we add experiments with PostgreSQL.
We conduct LHS sampling to collect 3000 observations under different configurations and select important knobs via SHAP based on the samples.
We analyze the top-5 important knobs in PostgreSQL.
And we find that the knob with the largest tunability, \textit{max\_worker\_processes} sets the maximum number of background processes the system can support, which shares a similar function with MySQL's top-1 important knob.
Beside, for  \textit{max\_worker\_processes} and \textit{shared\_buffers}, configuring larger values than the default can contribute to the decreasing of latency, which is also on par with the ones on MySQL.


Then, we compare the optimizers for workload JOB  over the top-5 and top-20 configuration spaces, respectively.
The conclusion is similar as on MySQL. 
SMAC achieves the best performance in both cases.
For the small space, mixed-kernel BO, one-hot BO, and vanilla BO demonstrate similar optimal results since there are no categorical knobs.
For medium space with categorical ones, mixed-kernel BO outperforms one-hot BO  and vanilla BO.
Overall, the BO-based methods outperform RL-based DDPG.
Due to space constraints, the detailed setup and results are presented in ~\autoref{app:pg} in Appendix.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}

\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{W2: }\textit{Section 5.1: The authors have chosen the top 5 and top 20 most important knobs according to their importance ranking algorithms. It is unclear why they discriminated their importance ranking in those two top raking lists.
}
\end{tcolorbox}
\noindent\textbf{Response: }
We agree it would be clearer to demonstrate the experiments on more subsets of different numbers of knobs, whilst the evaluation cost would have grown prohibitively high.
Therefore, based on the related work of black-box optimization~\cite{Eggensperger2013TowardsAE}, we choose three  representative configuration spaces with different sizes: small, medium, and large with dimensions of 5, 20, and 197(all) respectively. 
We have discussed the classification in \autoref{sec:exp2-setup} (Which optimizer is the winner) in the original paper.
We agree that it is confusing for the reader when reading  \autoref{sec:exp1-setup} (How to determine tuning knobs). 
In the revised manuscript, we move the justification about why to choose top-5 and top-20 most important knobs to the beginning of \autoref{sec:exp-tuning}:
\blue{``According to the proprieties of black-box optimization~\cite{Eggensperger2013TowardsAE}\ldots ranked by the importance measurement, respectively.''}

% Evaluating the  enumeration for all the subset of knobs ranking generated by different importance measurements are  expensive.
% We classify the configuration space into three sizes: small, large, medium  where we tune the most important 5, 20, and 197
% (all) knobs.
% We have discussed the classification in \autoref{sec:exp2-setup} in the original paper:
% ``According to the proprieties of black-box optimization~\cite{Eggensperger2013TowardsAE}, we
% choose three configuration spaces with different sizes: small,
% medium, and large, where we tune the most important 5, 20, and 197 (all) knobs ranked by SHAP, respectively.''


% We agree that it is confusing for the reader when reading  \autoref{sec:exp1-setup}. 
% We move the justification about why to choose top-5 and top-20 most important knobs to \autoref{sec:exp-tuning} in the revised manuscript:
% \blue{According to the proprieties of black-box optimization~\cite{Eggensperger2013TowardsAE}\ldots ranked by the importance measurement, respectively}


In addition, in the revised manuscript, we use the tuning benchmark via surrogates to evaluating the  enumeration for all the subset of knobs ranking and obtain similar conclusions about the performance importance measurements.
More details can be found in \autoref{sec8}.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{C1: }\textit{For completeness, I suggest adding the top 5 (or top 20) configuration parameters selected by SHAP. This information would be particularly useful to a database practitioner who is interesting in database tuning.
}
\end{tcolorbox}
\noindent\textbf{Response: }
Thanks for the suggestion.
As suggested by the reviewer, we add the top 20 configuration parameters selected by SHAP in Table \ref{tab:appendix-knob}  in Appendix and analyze their impact in \autoref{app-knob}.
We observe that configuring the maximum number of threads and the size of the log file can contribute to the performance the most, which is aligned with the previous analysis ~\cite{DBLP:conf/sigmod/AkenPGZ17,DBLP:conf/sigmod/ZhangWCJT0Z021,DBLP:journals/pvldb/AkenYBFZBP21}.
And 11 of the top-10 knobs are related to memory allocation, which indicates that the default setting of memory allocation in MySQL  may not be appropriate across the workloads and hardware.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{C2: }\textit{Section 8: "We observe that our tuning benchmark yields evaluation results closer to the result in Figure 10" - it should be Figure 7.
}
\end{tcolorbox}
\noindent\textbf{Response: }
We fix the reference issue in the revised manuscript.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}



\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{C3: }\textit{Section 8: ``For example, we can fit a surrogate with all the knobs as input to benchmark the knob selection modules''. 
It is not clear why you cannot already use the current benchmark for the knob selection modules since the 6250 samples were collected across all possible values over the 197-dimensional space.}
\end{tcolorbox}
\noindent\textbf{Response: }
We leave the knob selection benchmark as future work, since the 6250 samples might be insufficient to fit a surrogate over the 197-dimensional space.
And the corresponding $R^2$ of the surrogate fitted on the 6250 samples is about 60\%.

During the revision, we collect additional samples and obtain a surrogate model with 87\% $R^2$.
We add the evaluation of benchmarking knob selection modules in \autoref{sec8} in the revised manuscript. 
And the corresponding discussion is added:
\blue{``In addition, using surrogates could enlarge the number of evaluation cases of tuning algorithms.
To achieve this goal, we collect samples over the large (197-dimensional) configuration space and fit a surrogate.
In the previous evaluation, we conduct experiments over three configuration spaces since evaluating the enumeration of all  dimensions is expensive.
And when evaluating the optimizers, we fix the importance measurement to be SHAP.
With the surrogate benchmark, we could conduct extensive experiments over all the dimensions of configuration spaces (from top-1 to top-197) and all the importance measurements.
Then, we conduct 11820 experiments (197 knob sets $\times$  5 importance measurements $\times$ 6 optimizers $\times$  2 workloads) to benchmark the \textit{knob selection} and \textit{configuration optimization}  modules.
Since the \textit{knob selection}  aims to prune the configuration space, we report its performance on 20 knob sets (top-1 to top-20). 
And we report the performance of optimizers on the 197 knob sets.
As shown in Figure \ref{fig:exp-bench2}, SHAP remains the best importance measurement, and ablation study has significant performance variance.
SMAC performs the best, followed by mixed-kernel BO.
The evaluation results further validate our conclusions.''}
\rule{\textwidth}{0.1pt}


==> R3.tex <==

  \section*{REVIEWER \#3}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D1(W1): }\textit{The proposed efficient database tuning benchmark via surrogates idea is very novel and could save a lot of time while evaluating tuning optimizers. However, it would be great to see the surrogate model take place under various setups, and the biggest change would be in different database systems (only MySQL is presented, Postgres could be another great experiment). Since different systems could induce discrepancies which will also affect the end result for the most optimal knobs, and the effect of each knob could potentially change under various systems and workloads. But I understand if this is too much to include in this work.
}
\end{tcolorbox}
\noindent\textbf{Response: }
As suggested by the reviewer,  we conduct the evaluation using the surrogate model to benchmark tuning PostgresSQL.
We first collect 3000 observation samples 
We fit two surrogate models based on RFs over the small and medium configuration space of JOB workload in PostgreSQL.
And the surrogate model is available online in our repository \footnote{\url{https://github.com/PKU-DAIR/KnobsTuningEA}}.
The details can be found in ~\autoref{app:pg-bench} in Appendix due to the space constraint of the paper.
As shown in Figures ~\ref{fig:pg_optimizer} and ~\ref{fig:pg_benchmark},  the tuning benchmark yields evaluation results closer to the ones obtained through time-consuming workload replay (Figure ~\ref{fig:pg_optimizer}).
The configuration space of PostgreSQL is quite different with MySQL in terms of knob meanings,  types,  names  and value ranges.
The results on PostgreSQL demonstrate that researchers can conduct algorithm analysis and comparison efficiently under various setups with the help of the tuning benchmark.
%In addition to tuning benchmarks via surrogate with PostgreSQL, we add the benchmarking of the \textit{knob selection}  and \textit{configuration optimization} modules over a large evaluation space.
%We collect samples over the large (197-dimensional) configuration space and fit a surrogate.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D2(W2): }\textit{In Section 4.1, the authors nicely show a table about all the workloads used in the paper. But it is unclear how representative these workloads are. It would be better to show if these workloads have been used in previous work. Also, it would be nice to provide more insight on how the characteristics in Table 4 affect the challenge level of tuning tasks.
}
\end{tcolorbox}
\noindent\textbf{Response: }
Our experiments use JOB, SYSBENCH, TPC-C, Twitter as target workloads and Smallbank, SIbench, Voter, Seats, and TATP as source workloads.
The target workloads haven been used by the previous works in database configuration tuning~\cite{DBLP:conf/sigmod/AkenPGZ17, DBLP:conf/sigmod/ZhangLZLXCXWCLR19, DBLP:journals/pvldb/LiZLG19,DBLP:conf/sigmod/ZhangWCJT0Z021}.
When constructing the source workloads, we mainly want to increase the diversity of source data and make sure none of the data for the target workloads appears in the source.
We rewrite the \textbf{Workloads} paragraph in \autoref{sec4} to explain the reasons for our workload selection:
\blue{``To answer \textbf{Q1} and \textbf{Q2}, we use an analytical workload JOB and a transactional workload SYSBENCH.
JOB contains 113 multi-joint queries with realistic and complex joins~\cite{DBLP:journals/pvldb/LeisGMBK015}.
SYSBENCH is a multi-threaded benchmark frequently used for database systems.
To answer \textbf{Q3}, we use three OLTP workloads (SYSBENCH, TPC-C and Twitter) as target workloads, which have been adopted in previous studies~\cite{DBLP:conf/sigmod/AkenPGZ17,DBLP:conf/sigmod/ZhangLZLXCXWCLR19, DBLP:conf/sigmod/ZhangWCJT0Z021}.
And we construct diverse source workloads, including  Smallbank, SIbench, Voter, Seats, and TATP.
%SYSBENCH has read-only (RO), write-only (WO) and read-write (RW) modes and we use the RW mode.
They cover various size and read-write ratios, as shown in  Table \ref{wkl}.''}


As suggested by the reviewer, we emphasize the representativeness of the target workloads in \autoref{sec:app-workload} in Appendix:
\blue{``When answering \textbf{Q1} and \textbf{Q2}, we analyze the tuning performances over OLTP and OLAP scenarios.
We  use an OLAP workload -- JOB and an OLTP workload -- SYSBENCH.
The reason is that the two workloads are often adopted in evaluating  database configuration tuning methods and involve the scenarios of an online transaction/analytical processing.
For example, JOB is adopted by QTune~\cite{DBLP:journals/pvldb/LiZLG19} and SYSBENCH is adopted by CDBTune~\cite{DBLP:conf/sigmod/ZhangLZLXCXWCLR19}, QTune~\cite{DBLP:journals/pvldb/LiZLG19} and ResTune~\cite{DBLP:conf/sigmod/ZhangWCJT0Z021}.
When conducting knowledge transfer experiments (\textbf{Q3}),\ldots
We choose three OLTP workloads -- SYSBENCH, TPC-C, Twitter as the target tuning workloads, which have been adopted in previous studies.
For example, OtterTune~\cite{DBLP:conf/sigmod/AkenPGZ17}, CDBTune~\cite{DBLP:conf/sigmod/ZhangLZLXCXWCLR19}, and ResTune~\cite{DBLP:conf/sigmod/ZhangWCJT0Z021}) has adopted TPC-C for evaluation and  ResTune has also adopted Twitter.''}

\begin{table}[h]
\caption{Performance of random samples over configuration space.}\label{tab:cover1}
\begin{tabular}{|c|c|c|}
\hline
                                          & SYSBENCH & JOB    \\ \hline
Better Than The Default                   & 14.34\%  & 5.28\% \\ \hline
Better Than 95\% of the Estimated Optimum & 0.56\%   & 0.12\% \\ \hline
\end{tabular}
\end{table}



As for the challenge level of the tuning task, we think the performance of random samples over the configuration space can be an indicator.
For example, if a large percentage of random samples have good performance, the tuning task is considered to be easy.
We summarize the performance of the 6250 random samples generated by LHS over the 197-dimensional configuration space  on SYSBENCH and JOB workloads.
Table \ref{tab:cover1} presents the result.
We observe that 14.34\% of the random samples are better than the default for SYSBENCH workload and  5.28\% for JOB workload, indicating the tuner has more chance to find configurations better than the default in SYSBENCH workload.

Due to the complex nature of the relationship between configurations and database performances, mapping the workload characteristics to the challenge level of tuning tasks remains an open problem.
Based on our initial observations, a more complex query workload might lead to a more challenging tuning task.
(JOB's queries contain multiple realistic and complex joins, while SYSBENCH's queries are relatively more straightforward.)
%In addition, we also add the benchmarking of knob selection 
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D3(W2): }\textit{In Section 5, GP and DDPG are used as underlying configuration optimization methods. It is unclear why only these 2 methods are tested. In Figure 3, it is clear to see that the choice of optimization methods will change the ranking of different importance measurements. I would suspect that if we use a different underlying optimization method, it might change the conclusion - “SHAP is the best importance measurement”.}

\noindent\textbf{D3:}\textit{ Justify on choosing GP and DDPG. The revision action can be either (1) to add a paragraph to explain the reason for using GP and DDPG or (2) to show a figure of 2 workloads on all the methods. It could be a box plot for the sake of limited space, where the box represents different underlying optimization methods.
}
\end{tcolorbox}
\noindent\textbf{Response: }
We agree that presenting the results on all the  underlying optimizers could improve the conclusion's credibility.
As suggested by the reviewer, we use box plots in Figure \ref{fig:exp1} to show the performance of different importance measurements over all the  optimizers.
In the original paper, we chose GP (vanilla BO) and DDPG  since they are two representatives of BO-based and RL-based methods.
As discussed in the original paper, we compare the importance measurements using the two optimizers to narrow down the size of search (evaluation) space.
``Because of the joint nature, the search space of the end-to-end optimization is complex and huge. 
In our evaluation, we decompose the joint space reasonably to narrow the search space. For example, when comparing the importance measurements, we fix the optimizers to the two representative ones, vanilla BO and DDPG.''

For the revised manuscript, we conduct additional experiments using the other six optimizers and  update the statistics in Table \ref{tab:imp-performance} accordingly.
We rewrite the corresponding setup in \autoref{sec:exp1-setup}:
\blue{``We perform configuration optimization on each knob set, using the eight optimizers in Table \ref{tab:algorithm}.
We collect the performance rankings of the importance measurements in terms of the best configuration found by each optimizer.''}

As shown in Table \ref{tab:imp-performance} in the revised manuscript, the conclusion that SHAP is the best importance measurement remains.
And the conclusions is similar, except that Lasso ranks the last and ablation analysis ranks the second to last. 
(When only two optimizers i.e., vanilla BO and DDPG are tested, ablation analysis ranks the last and Lasso  ranks the second to last.)
The new result over all the optimizers is consistent with the fact that Lasso assumes linear or quadratic configuration spaces, failing to model the complex dependencies from configurations to database performance.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D4(W2): }\textit{D4. (W2) In Section 7, SYSBENCH, TPC-C, and Twitter are used as target workloads. It is unclear why these 3 are picked as the target. Also, it is unclear why SIBench is not a target workload, since it is in a different class. It would be better to explain what makes it difficult to transfer knowledge to them.
}
\end{tcolorbox}
\noindent\textbf{Response: }
We attempt  to imitate cloud environments where there are various and diverse historical workloads as source workloads.
And a tuning task for an unseen target workload is initialized by the users.
We adopt SYSBENCH, TPC-C, and Twitter since they  are target workloads adopted by previous studies~\cite{DBLP:conf/sigmod/AkenPGZ17,DBLP:conf/sigmod/ZhangLZLXCXWCLR19, DBLP:conf/sigmod/ZhangWCJT0Z021}, as the response to \textbf{D2}.
% And we do not claim that transferring knowledge to the three workloads is more difficult.
When constructing the source workloads, we make sure that the target workloads are held out and try to provide diverse source workloads as in the cloud. 
SIBench has limited tuning  opportunities and we add it into the source workloads to increase the diversity.
The detailed modifications are as follows.


We rewrite the description  in \autoref{sec4} to briefly explain why the three target workloads are adopted:
\blue{``To answer \textbf{Q3}, we adopt three OLTP workloads (SYSBENCH, TPC-C and Twitter) as target workloads, which have been adopted in previous studies~\cite{DBLP:conf/sigmod/AkenPGZ17,DBLP:conf/sigmod/ZhangLZLXCXWCLR19, DBLP:conf/sigmod/ZhangWCJT0Z021}.''}
And in \autoref{sec:app-workload} in Appendix, we further discuss why we focus on transferring between OLTP workloads and emphasis the repressiveness of the chosen target workloads:
\blue{``When conducting knowledge transfer experiments (\textbf{Q3}), we focus on the OLTP scenarios since there are fewer OLAP workloads suitable for constructing  source workloads of tuning tasks, except JOB and TPC-H.
We choose three OLTP workloads -- SYSBENCH, TPC-C, Twitter as the target tuning workloads, which have been adopted in previous studies.
For example, OtterTune~\cite{DBLP:conf/sigmod/AkenPGZ17}, CDBTune~\cite{DBLP:conf/sigmod/ZhangLZLXCXWCLR19}, and ResTune~\cite{DBLP:conf/sigmod/ZhangWCJT0Z021}) has adopted TPC-C for evaluation and  ResTune has also adopted Twitter.''}



SIBench is is a microbenchamark designed to explore snapshot isolation in DBMSs~\cite{DBLP:journals/pvldb/JungHFR11}.
Based on our observations, the tuning opportunities for SIBench are limited.
The performance of the default configuration on SIbench is 230 \#txn/s, and the best performance optimized by DDPG over 300 iterations is 243 \#txn/s.
We add SIBench to the source workloads to increase the diversity.
We discuss the construction of source workloads in \autoref{sec4}: \blue{``And we construct diverse source workloads, including  Smallbank, SIbench, Voter, Seats, and TATP.
They cover various size and read-write ratios, as shown in  Table \ref{wkl}.''}
We add the detailed discussion in \autoref{sec:app-workload} in Appendix:
\blue{
``We use additional four OLTP workloads (i.e., SEATS, Smallbank, TATP, Voter, SIBENCH) as source workloads and configure them with various sizes, read-write ratios as shown in Table ~\ref{wkl}.
SIBench is a microbenchmark designed to explore snapshot isolation in DBMSs~\cite{DBLP:journals/pvldb/JungHFR11}.
Based on our observations, the tuning opportunity for SIBench is limited.
We add SIBench to the source workloads with the purpose of increasing the diversity.''}
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D5(W3) : }\textit{This paper is very insightful. And the micro evaluation is comprehensive. But it would be nice to have an end-to-end evaluation of the 7 methods before diving into the modules. If there is an existing macro evaluation, it would be better to refer to their conclusion.
}
\end{tcolorbox}
\noindent\textbf{Response: }
As suggested by the reviewer, we refer to a recent evaluation~\cite{DBLP:journals/pvldb/AkenYBFZBP21} that compares CDBTune (DDPG) and OtterTune (GP) in \autoref{sec:exp2-performance}.
Its conclusion is consistent with our results that CDBTune takes longer to converge.
\blue{``We also notice that the tuning cost of DDPG is constantly high due to the requirement of learning a great number of neural network parameters,  which is consistent with the existing evaluation~\cite{DBLP:journals/pvldb/AkenYBFZBP21}.''}


We break down existing tuning methods, and compare possible design ``paths'' across the intra-algorithm choices.
Many database configuration tuning methods~\cite{ DBLP:conf/sigmod/ZhangLZLXCXWCLR19,DBLP:journals/pvldb/LiZLG19,DBLP:conf/sigmod/KunjirB20, DBLP:journals/pvldb/DuanTB09} focus on \textit{configuration optimization} module and their tuning knobs are selected by DBAs not made public.
It is hard to conduct a fair and comprehensive end-to-end evaluation, covering all the existing tuning systems.
%In order to conduct a 
Therefore, we abstract the underlying technologies of existing tuning systems and compare the possible design ``paths'', considering the choices of technologies for \textit{knob selection}, \textit{configuration optimization} and \textit{knowledge transfer}.


There do exist other end-to-end evaluations, covering some tuning systems in previous studies.
But the end-to-end performance could be contributed to  new modules or  designs tailored for new scenarios. 
For example, OtterTune has demonstrated better performance than iTuned, since OtterTune is equipped with workload mapping that transfers historical knowledge.
%But most evaluations are conducted on new scenarios.
And QTune proposes query-level and cluster-level tuning and has demonstrated better performances than the previous systems (CDBTune and OtterTune) in the two scenarios.
ResTune proposes resource-oriented tuning and has demonstrated better performances than CDBTune and OtterTune when optimizing with constraints.
%In addition, conflict results exist.
%CDBTune is shown to be superior to OtterTune in its evaluation.
%But a recent evaluation shows that OtterTune performs better than DDPG (CDBTune) in most cases, which is consistent with our evaluation.
\newline
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}


\noindent\begin{tcolorbox}[colback=gray!10,%gray background
                  arc=0mm, auto outer arc,
                  boxrule=0pt,
                  nobeforeafter,
                  boxsep=0.5pt
                 ]
\noindent\textbf{D6: }\textit{In terms of presentation, (1) Table 4 and 5 can be split into sections accordingly since the workloads and instances are not used throughout the paper. Section 5 and 6 are using the same setup and are different from Section 7. The overlap is very small. (2) There are also typos to fix, such as missing space between words. For example, “(action). However,” in para2 of p10. “SHAP is the best importance measurements” in Sec 5.4. (3) In Section 3.1, knob selection is discussed. It would be nice to formulate the knob selection problem beforehand. Because the terminology is inconsistent where “feature” is “knob”. It is unclear if the knob selection problem is the same as feature selection for a regression model.
}
\end{tcolorbox}
\noindent\textbf{Response: }
Thanks for the suggestions. 
As suggested by the reviewer, we make the following modifications.
\begin{itemize}
    \item 
    We split Table 4 in the original paper into sections accordingly.
    We explicitly state that the target database system is deployed in an instance with 8 vCPUs and 16 GB RAM in \autoref{sec4} (General setup of evaluation).
    And in \autoref{sec:exp-transfer} (Can we transfer knowledge to speed up the target tuning task),  we supplement that we have used more hardware configurations for database instances  and refer to the  Table \ref{tab:hardware} in \autoref{app-knob} in Appendix for the specific setting.
    In addition, we rewrite the \textbf{Workloads}  paragraph in  \autoref{sec4} to  interpret Table 5 in the original paper (Table \ref{wkl} in the revised manuscript) clearly.
    We state that SYSBENCH and JOB are used in ~\autoref{sec5} and ~\autoref{sec6}, and all the workloads expect JOB are used in ~\autoref{sec:exp-transfer} for knowledge transfer. 
     
    \item We have checked the manuscripts carefully and fixed the corresponding typos.
    \item We make the terminology in \autoref{sec:men-knob} consistent and replace the ``features'' with ``knobs''. 
    For variance-based measurements, knob selection is the same as feature selection for a regression model since we need to select knobs with largest impact on the objective variables.
    For tunability-based measurements, the knob selection problem is different from feature selection for regression.
\end{itemize}
\rule{\textwidth}{0.1pt}
\vspace{0.5pt}
